Learning to Represent and Predict Sets with Deep Neural Networks

In this thesis, we develop various techniques for working with sets in machine learning. Each input or output is not an image or a sequence, but a set: an unordered collection of multiple objects, each object described by a feature vector. Their unordered nature makes them suitable for modeling a wide variety of data, ranging from objects in images to point clouds to graphs. Deep learning has recently shown great success on other types of structured data, so we aim to build the necessary structures for sets into deep neural networks. The first focus of this thesis is the learning of better set representations (sets as input). Existing approaches have bottlenecks that prevent them from properly modeling relations between objects within the set. To address this issue, we develop a variety of techniques for different scenarios and show that alleviating the bottleneck leads to consistent improvements across many experiments. The second focus of this thesis is the prediction of sets (sets as output). Current approaches do not take the unordered nature of sets into account properly. We determine that this results in a problem that causes discontinuity issues with many set prediction tasks and prevents them from learning some extremely simple datasets. To avoid this problem, we develop two models that properly take the structure of sets into account. Various experiments show that our set prediction techniques can significantly benefit over existing approaches.

==> chapters/learn-to-count/tikz.tex <==
\usepackage{tikz}
\usepackage{amssymb}
\usepackage{xcolor}

\usetikzlibrary{fit, positioning, calc}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{backgrounds}


\definecolor{yes}{RGB}{0, 0, 0}
\definecolor{no}{RGB}{255, 255, 255}
\definecolor{maybe}{RGB}{128, 128, 128}  % Averaged in LAB space
\definecolor{grey}{RGB}{224, 224, 224}
\definecolor{bg}{RGB}{250, 250, 250}
\definecolor{blue}{HTML}{004CDB}
\definecolor{lblue}{HTML}{74c9e5}
\definecolor{red}{HTML}{FF4500}
\definecolor{yellow}{HTML}{FFb31a}
\definecolor{ccc1}{HTML}{3a913a}
\definecolor{ccc2}{HTML}{c03c3d}
\definecolor{ccc3}{HTML}{9371b2}
\definecolor{ccc4}{HTML}{e0802c}
\definecolor{cc1}{HTML}{1fad1f}
\definecolor{cc2}{HTML}{d42525}
\definecolor{cc3}{HTML}{9446dd}
\definecolor{cc4}{HTML}{ee8020}
\colorlet{c1}{cc1!80!white}
\colorlet{c2}{cc2!80!white}
\colorlet{c3}{cc3!80!white}
\colorlet{c4}{cc4!80!white}


\makeatletter
\newsavebox{\measure@tikzpicture}
\tikzset{
    every picture/.append style={x=1.5cm, y=1.5cm},
    ledge/.style={->, >=stealth, loop, looseness=7},
    dedge/.style={<->, >=stealth},
    sedge/.style={->, >=stealth},
    imedge/.style={->, >=stealth, draw=yellow},
    node/.style={circle, draw, fill=grey},
    varname/.style={midway, above, opacity=1},
    object/.style={rounded corners=0.8em, draw, dotted, inner sep=1em, fill=bg},
    box/.style={% only the fill and draw styles
        draw=yellow, line width=0.35mm},
    block rect/.style={% fill, draw + rectangle (without measurements)
        box, rectangle},
    block/.style={% fill, draw, rectangle + minimum measurements
        block rect, minimum height=0.8cm, minimum width=6em},
    from/.style args={#1 to #2}{% without transformations
        above right={0cm of #1},% needs positioning library
        /utils/exec=\pgfpointdiff
            {\tikz@scan@one@point\pgfutil@firstofone(#1)\relax}
            {\tikz@scan@one@point\pgfutil@firstofone(#2)\relax},
        minimum width/.expanded=\the\pgf@x,
        minimum height/.expanded=\the\pgf@y},
    w/.style = {circle, draw, fill=white, inner sep=0mm, minimum size=3.5mm, thick},
    params/.style = {rectangle, rounded corners=1mm, draw, fill=lblue, inner sep=1mm, thick},
    no params/.style = {rectangle, rounded corners=1mm, draw, fill=grey, inner sep=1mm, thick},
    nodes/.pic={
        \node [node, fill=yes] (tl) at (0, 0) {};
        \node [node, fill=no] (tr) at (0, -1) {};
        \node [node, fill=yes] (bl) at (1, 0) {};
        \node [node, fill=yes] (br) at (1, -1) {};

        \begin{scope}[on background layer]
            \node [object, fit=(bl) (br)] {};
            \node [object, fit=(tl)] {};
            \node [object, fit=(tr)] {};
        \end{scope}
    },
    a/.pic={
        \pic {nodes};
        \coordinate (aux1) at ($(tl)!0.46!(tr)$);
        \coordinate (aux2) at ($(tl)!0.54!(tr)$);
        \node at (-2, -0.5)  {
            \includegraphics[width=3.5cm]{COCO_val2014_000000121112}
        };
        \node (c11) [box, from={-1.55,-0.66 to -0.97,-0.13}] {};
        \node (c12) [box, from={-1.59,-0.70 to -0.93, -0.09}] {};
        \node (c2) [box, from={-2.72,-0.70 to -2.22, -0.16}] {};
        \node (k) [box, from={-2.45,-1.22 to -0.859, -0.83}] {};
        \draw [imedge] (k.east |- tr) to[out=0, in=180] (tr);
        \draw [imedge] (c2) to[out=45, in=180, looseness=0.3] (tl);
        \draw [draw=yellow] (c11.east |- aux1) to[out=0, in=180] (aux1);
        \draw [draw=yellow] (c12.east |- aux2) to[out=0, in=180] (aux2);
        \draw [imedge] (aux1) to[out=0, in=225] (bl);
        \draw [imedge] (aux2) to[out=0, in=135] (br);
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m a$};
    },
    A/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m A$};

        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
        \draw [dedge] (bl) -- (br);

        \draw [in=180, out=90, ledge] (tl) to (tl);
        \draw [in=0, out=90, ledge] (bl) to (bl);
        \draw [in=0, out=-90, ledge] (br) to (br);
    },
    Acolor/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m A$};

        \draw [dedge, draw=blue] (tl) -- (bl);
        \draw [dedge, draw=blue] (tl) -- (br);
        \draw [dedge, draw=red] (bl) -- (br);

        \draw [in=180, out=90, ledge] (tl) to (tl);
        \draw [in=0, out=90, ledge] (bl) to (bl);
        \draw [in=0, out=-90, ledge] (br) to (br);
    },
    O/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m D$};

        \draw [dedge] (tl) -- (tr);
        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
        \draw [dedge] (tr) -- (bl);
        \draw [dedge] (tr) -- (br);
        \node [node, fill=yes] at (0, -1) {};
    },
    B/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\tilde{\m A}$};

        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
    },
    Bprime/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\tilde{\m A}'$};

        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
        \draw [in=180, out=90, ledge] (tl) to (tl);
        \draw [in=0, out=90, ledge] (bl) to (bl);
        \draw [in=0, out=-90, ledge] (br) to (br);
    },
    s/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m s$};

        \node [node, fill=yes] at (0, -1) {};
        \node [node, fill=maybe] at (1, 0) {};
        \node [node, fill=maybe] at (1, -1) {};
    },
    C/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m C$};
        \node [node, fill=maybe] at (1, 0) {};
        \node [node, fill=maybe] at (1, -1) {};

        \draw [in=180, out=90, ledge, draw=yes] (tl) to (tl);
        \draw [in=0, out=90, ledge, draw=maybe] (bl) to (bl);
        \draw [in=0, out=-90, ledge, draw=maybe] (br) to (br);

        \draw [dedge, draw=maybe] (tl) -- (bl);
        \draw [dedge, draw=maybe] (tl) -- (br);
    },
    C2/.pic={
        \node [node, fill=yes] (tl) at (0, 0) {};
        \node [node, fill=no, opacity=0] (tr) at (1, 0) {};
        \node [node, fill=no] (bl) at (0, -1) {};
        \node [node, fill=no, opacity=0] (br) at (1, -1) {};
        \node [node, fill=yes] (bm) at (1, -0.5) {};

        \begin{scope}[on background layer]
            \node [object, fit=(tr) (br)] {};
            \node [object, fit=(tl)] {};
            \node [object, fit=(bl)] {};
        \end{scope}

        \draw [in=180+22.5, out=90+22.5, ledge, draw=yes] (tl) to (tl);
        \draw [in=0+22.5, out=-90+22.5, ledge, draw=yes] (bm) to (bm);

        \draw [dedge] (tl) -- (bm);
    },
    model/.pic={
        \node (img) {Image};
        \node (detect) [params, right = 5 mm of img, text width=1.6cm, align=center] {R-CNN};
        \node (l2) [no params, right = 3 mm of detect] {\tiny L2 norm};

        \node (quest) [below = 2 cm of img] {Question};
        \node (embed) [params, text width=1.6cm, align=center] at (detect |- quest) {Embedding};
        \node (rnn) [params, align=center] at (l2 |- embed) {GRU};

        \coordinate (atttop) at ($(l2)!0.25!(rnn)$);
        \coordinate (attmid) at ($(l2)!0.5!(rnn)$);
        \coordinate (attbottom) at ($(l2)!0.75!(rnn)$);
        \coordinate (attmid) at ($(l2)!0.5!(rnn)$);
        \node (attfuse) [no params, right = 7 mm of attmid] {\LARGE$\diamond$};
        \node (attw) [w, right = 2 mm of attfuse] {w};
        \coordinate (softpos) at (attw |- atttop);
        \node (softmax) [no params, right = 7 mm of softpos] {\tiny softmax};
        \node (sum) [no params] at (softmax |- l2) {\tiny$\sum$};

        \coordinate (wq) at (sum.east |- rnn);
        \coordinate (classmiddle) at (sum |- attmid);
        \node (classfuse) [no params, right = 8 mm of classmiddle] {\LARGE$\diamond$};
        \node (classadd) [no params, right = 2 mm of classfuse, draw=red] {\tiny $+$};
        \node (classbn) [params, right = 2 mm of classadd] {\scriptsize BN};
        \node (class) [w, right = 2 mm of classbn] {w};
        \node (classsoft) [no params, right = 2 mm of class] {\tiny softmax};
        \node (end) [right = 2 mm of classsoft] {};

        \node (abovesum) [above = 7 mm of sum] {};
        \node (count) [params, draw=red] at ([xshift=3mm]abovesum) {Count};
        \node (bn) [params, draw=red] at (classadd |- atttop) {\scriptsize BN};
        \node (relu) [no params, draw=red] at (classadd |- sum) {\tiny ReLU};


        \draw [thick, sedge] (img) to ([xshift=-1mm]detect.west);
        \draw [sedge] (detect) to (l2) to (sum);
        \draw [thick, sedge] (quest) to ([xshift=-1mm]embed.west);
        \draw (embed) to (rnn) to (wq);
        \draw (classfuse) to (classadd) to (classbn) to (class) to (classsoft) [sedge] to (end);
        \draw [ledge, out=-45, in=-135, looseness=4] (rnn) to (rnn);

        \draw [sedge] (l2.east) to [out=0, in=90] node [pos=0.5, w] {w} (attfuse);
        \draw [sedge] (rnn.east) to [out=0, in=-90] node [pos=0.5, w] {w} (attfuse);
        \draw (attfuse) to (attw);
        \draw ([yshift=0.3mm]attw.east) to [out=0, in=-90] ([xshift=-0.3mm]softmax.south);
        \draw ([yshift=-0.3mm]attw.east) to [out=0, in=-90] ([xshift=0.3mm]softmax.south);
        \draw [sedge] ([xshift=-0.3mm]softmax.north) to ([xshift=-0.3mm]sum.south);
        \draw [sedge] ([xshift=0.3mm]softmax.north) to ([xshift=0.3mm]sum.south);

        \draw [sedge] (sum) to [out=0, in=90] node [pos=0.5, w] {w} (classfuse);
        \draw [sedge] (wq) to [out=0, in=-90] node [pos=0.5, w] {w} (classfuse);

        \draw [color=red] (count) to [out=0, in=90] node [pos=0.5, color=black, draw=red, w] {w} (relu);
        \draw [color=red] (relu) to (bn) [sedge] to (classadd);

        \begin{scope}[on background layer]
            \draw [sedge, color=red] ([yshift=0.3mm]attw.east) to [out=0, in=180, looseness=0.8] node [pos=0.7, color=black, draw=red, no params] {\small$\sigma$} ([yshift=-0.3mm]count.west);
            \draw [sedge, color=red] ([xshift=-0.4mm, yshift=-0.4mm]detect.north east) to [out=45, in=180, looseness=0.8] node [pos=0.5, above, rotate=13] {\tiny bounding boxes only} ([yshift=0.3mm]count.west);
            \coordinate (crossmid) at ($(attw)!0.4!(count)$);
            \node [fill=white, inner sep=0.8mm, text width=1cm] at (crossmid |- l2) { };
        \end{scope}

    },
    model2/.pic={
        \clip (-0.5, -1.4) rectangle (7.4, 0.25);
        \node (img) {Image};
        \node (detect) [params, right = 7 mm of img, text width=1.6cm, align=center] {R-CNN};

        \node (quest) [below = 1.2 cm of img] {Question};
        \node (rnn) [params, text width=1.6cm, align=center] at (detect |- quest) {RNN};

        \coordinate (atttop) at ($(detect)!0.25!(rnn)$);
        \coordinate (attmid) at ($(detect)!0.5!(rnn)$);
        \coordinate (attbottom) at ($(detect)!0.75!(rnn)$);
        \node (attfuse) [no params, right = 9 mm of attmid] {\small$\diamond$};
        \node (attw) [params, right = 2 mm of attfuse] {Attention};
        \coordinate (softpos) at (attw |- atttop);
        \node (sum) [no params, scale=0.9] at ([xshift=13mm]attw |- detect) {\tiny$\sum$};

        \coordinate (wq) at (sum.east |- rnn);
        \coordinate (classmiddle) at (sum |- attmid);
        \node (classfuse) [no params, right = 8 mm of classmiddle] {\small$\diamond$};
        \node (classmlp) [params, right = 2 mm of classfuse] {MLP};
        \node (end) [right = 3 mm of classmlp, text width = 3 cm, scale=0.75] {Classify answer\\from 3000 most common answers};

        \node (abovesum) [above = 7 mm of sum] {};

        \draw [thick, sedge] (img) to ([xshift=-1mm]detect.west);
        \draw [sedge] (detect) to (sum);
        \draw [thick, sedge] (quest) to ([xshift=-1mm]rnn.west);
        \draw (rnn) to (wq);
        \draw (classfuse) to (classmlp) [sedge] to (end);
        \draw [ledge, out=45, in=135, looseness=4] (rnn) to (rnn);

        \draw [sedge] (detect.east) to [out=0, in=90] (attfuse);
        \draw [sedge] (rnn.east) to [out=0, in=-90] (attfuse);
        \draw (attfuse) to (attw);
        \draw [sedge] (attw.east) to [out=0, in=-90] (sum.south);

        \draw [sedge] (sum) to [out=0, in=90] (classfuse);
        \draw [sedge] (wq) to [out=0, in=-90] (classfuse);
        %\draw [brown] (current bounding box.south west) rectangle (current bounding box.north east);
    },
    dummyimg/.pic={
        \node [fill=black, inner sep = 0.5cm] (bg) at (0, 0) {};
        \node [below right = 4mm and 1mm of bg.north west, color=white, inner sep = 0.3mm, box] (star) {$\bigstar$};
    },
    fv/.pic={
        \node [rectangle, draw=black, thick, minimum size = 3mm, fill=c1] at (0, 0) {};
        \node [rectangle, draw=black, thick, minimum size = 3mm, fill=c2] at (0.2, 0) {};
        \node [rectangle, draw=black, thick, minimum size = 3mm, fill=c3] at (0.4, 0) {};
        \node [rectangle, draw=black, thick, minimum size = 3mm, fill=c4] at (0.6, 0) {};
    },
    probs/.pic={
        \node (img1) {\begin{tikzpicture}\pic{dummyimg};\end{tikzpicture}};
        \node [below = 0 mm of img1] (img2) {\begin{tikzpicture}\pic{dummyimg};\end{tikzpicture}};
        \node [below = 3.65mm of img2.center] (img3) {\begin{tikzpicture}\pic{dummyimg};\end{tikzpicture}};

        \node [left = 0mm of img1] {Image 1};
        \coordinate (img25) at ($(img2.west)!0.5!(img3.west)$);
        \coordinate (img26) at ($(img2.west)!0.2!(img3.west)$);
        \coordinate (img24) at ($(img2.west)!0.8!(img3.west)$);
        \node [left = 0mm of img25] {Image 2};

        \node [inner sep=0mm, right = 4mm of img1] (fv1) {\begin{tikzpicture}\pic{fv};\end{tikzpicture}};
        \node [inner sep=0mm,] (fv2) at (fv1 |- img26) {\begin{tikzpicture}\pic{fv};\end{tikzpicture}};
        \node [inner sep=0mm,] (fv3) at (fv1 |- img24) {\begin{tikzpicture}\pic{fv};\end{tikzpicture}};
        \coordinate (fv) at ($(fv1)!0.5!(fv3)$);

        \node [right = 2.5cm of fv1] (w1) {$w$};
        \node [right = 2.5cm of fv2] (w2) {$w$};
        \node [right = 2.5cm of fv3] (w3) {$w$};

        \draw [sedge] (fv1) -- (w1);
        \draw [sedge] (fv2) -- (w2);
        \draw [sedge] (fv3) -- (w3);

        \node [params, right = of fv, minimum height = 3cm] (att1) {Attention};

        \node [right = 10mm of w1] (v1) {$1.0$};
        \node [right = 10mm of w2] (v2) {$0.5$};
        \node [right = 10mm of w3] (v3) {$0.5$};

        \draw [sedge] (w1) -- (v1);
        \draw [sedge] (w2) -- (v2);
        \draw [sedge] (w3) -- (v3);

        \node [no params, right = 3.85cm of fv, anchor=north, rotate=-90, anchor=south,  minimum width = 3cm] (softm) {Softmax};

        \coordinate (v25) at ($(v2.east)!0.5!(v3.east)$);
        \node [no params, right = 3mm of v1, minimum height=1cm] (s1) {$\sum$};
        \node [no params, right = 3mm of v25, minimum height=1cm] (s2) {$\sum$};

        \draw [sedge] (v1) -- (s1);
        \draw [sedge] (v2) -- (s2.west |- v2);
        \draw [sedge] (v3) -- (s2.west |- v3);

        \node [right = 4mm of s1, inner sep=0mm] (out1) {\begin{tikzpicture}\pic{fv};\end{tikzpicture}};
        \node [right = 4mm of s2, inner sep=0mm] (out2) {\begin{tikzpicture}\pic{fv};\end{tikzpicture}};

        \coordinate (s15) at ($(s1)!0.5!(s2)$);
        \node (eq) at (out1 |- s15) {\small$=$};

        \draw [sedge] (s1) -- (out1);
        \draw [sedge] (s2) -- (out2);

        \node [above = 2mm of fv1, rotate=-90, anchor=center, scale=1.3, inner sep=0mm] (to) {$\Bigg\{$};
        \node [below = 2mm of fv1, rotate=-90, anchor=center, scale=1.3, inner sep=0mm] {$\Bigg\}$};
        \node [above = 2mm of fv2, rotate=-90, anchor=center, scale=1.3, inner sep=0mm] {$\Bigg\{$};
        \node [below = 2mm of fv3, rotate=-90, anchor=center, scale=1.3, inner sep=0mm] (bo) {$\Bigg\}$};

        \draw [sedge] (to.west) to[bend left=20] (s1.north west);
        \draw [sedge] (bo.east) to[bend right=20] (s2.south west);

        \draw [draw=yellow, sedge] (0, -0.06) to[in=180, out=0] (fv1);
        \draw [draw=yellow, sedge] (0, -0.89) to[in=180, out=0] (fv2);
        \draw [draw=yellow, sedge] (0, -1.55) to[in=180, out=0] (fv3);
    },
}
\makeatother


==> chapters/learn-to-count/workshop/tikz.tex <==
\usepackage{tikz}

\usetikzlibrary{fit, positioning, calc}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{backgrounds}

\definecolor{yes}{RGB}{0, 0, 0}
\definecolor{no}{RGB}{255, 255, 255}
\definecolor{maybe}{RGB}{128, 128, 128}  % Averaged in LAB space
\definecolor{grey}{RGB}{224, 224, 224}
\definecolor{bg}{RGB}{250, 250, 250}
\definecolor{blue}{HTML}{004CDB}
\definecolor{lblue}{HTML}{b2cdff}
\definecolor{red}{HTML}{FF4500}
\definecolor{yellow}{HTML}{FFb31a}

\makeatletter
\newsavebox{\measure@tikzpicture}
\tikzset{
    every picture/.append style={x=1.5cm, y=1.5cm},
    ledge/.style={->, >=stealth, loop, looseness=7},
    dedge/.style={<->, >=stealth},
    sedge/.style={->, >=stealth},
    imedge/.style={->, >=stealth, draw=yellow},
    node/.style={circle, draw, fill=grey},
    varname/.style={midway, above, opacity=1},
    object/.style={rounded corners=0.8em, draw, dotted, inner sep=1em, fill=bg},
    box/.style={% only the fill and draw styles
        draw=yellow, line width=0.35mm},
    block rect/.style={% fill, draw + rectangle (without measurements)
        box, rectangle},
    block/.style={% fill, draw, rectangle + minimum measurements
        block rect, minimum height=0.8cm, minimum width=6em},
    from/.style args={#1 to #2}{% without transformations
        above right={0cm of #1},% needs positioning library
        /utils/exec=\pgfpointdiff
            {\tikz@scan@one@point\pgfutil@firstofone(#1)\relax}
            {\tikz@scan@one@point\pgfutil@firstofone(#2)\relax},
        minimum width/.expanded=\the\pgf@x,
        minimum height/.expanded=\the\pgf@y},
    w/.style = {circle, draw, fill=white, inner sep=0mm, minimum size=3.5mm, thick},
    params/.style = {rectangle, rounded corners=1mm, draw, fill=lblue, inner sep=1mm, thick},
    no params/.style = {rectangle, rounded corners=1mm, draw, fill=grey, inner sep=1mm, thick},
    nodes/.pic={
        \node [node, fill=yes] (tl) at (0, 0) {};
        \node [node, fill=no] (tr) at (0, -1) {};
        \node [node, fill=yes] (bl) at (1, 0) {};
        \node [node, fill=yes] (br) at (1, -1) {};

        \begin{scope}[on background layer]
            \node [object, fit=(bl) (br)] {};
            \node [object, fit=(tl)] {};
            \node [object, fit=(tr)] {};
        \end{scope}
    },
    a/.pic={
        \pic {nodes};
        \coordinate (aux1) at ($(tl)!0.46!(tr)$);
        \coordinate (aux2) at ($(tl)!0.54!(tr)$);
        \node at (-2, -0.5)  {
            \includegraphics[width=0.25\linewidth]{../COCO_val2014_000000121112}
        };
        \node (c11) [box, from={-1.55,-0.66 to -0.97,-0.13}] {};
        \node (c12) [box, from={-1.59,-0.70 to -0.93, -0.09}] {};
        \node (c2) [box, from={-2.72,-0.70 to -2.22, -0.16}] {};
        \node (k) [box, from={-2.45,-1.22 to -0.859, -0.83}] {};
        \draw [imedge] (k.east |- tr) to[out=0, in=180] (tr);
        \draw [imedge] (c2) to[out=45, in=180, looseness=0.3] (tl);
        \draw [draw=yellow] (c11.east |- aux1) to[out=0, in=180] (aux1);
        \draw [draw=yellow] (c12.east |- aux2) to[out=0, in=180] (aux2);
        \draw [imedge] (aux1) to[out=0, in=225] (bl);
        \draw [imedge] (aux2) to[out=0, in=135] (br);
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m a$};
    },
    A/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m A$};

        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
        \draw [dedge] (bl) -- (br);

        \draw [in=180, out=90, ledge] (tl) to (tl);
        \draw [in=0, out=90, ledge] (bl) to (bl);
        \draw [in=0, out=-90, ledge] (br) to (br);
    },
    Acolor/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m A$};

        \draw [dedge, draw=blue] (tl) -- (bl);
        \draw [dedge, draw=blue] (tl) -- (br);
        \draw [dedge, draw=red] (bl) -- (br);

        \draw [in=180, out=90, ledge] (tl) to (tl);
        \draw [in=0, out=90, ledge] (bl) to (bl);
        \draw [in=0, out=-90, ledge] (br) to (br);
    },
    O/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m D$};

        \draw [dedge] (tl) -- (tr);
        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
        \draw [dedge] (tr) -- (bl);
        \draw [dedge] (tr) -- (br);
    },
    B/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\tilde{\m A}$};

        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
    },
    Bprime/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\tilde{\m A}'$};

        \draw [dedge] (tl) -- (bl);
        \draw [dedge] (tl) -- (br);
        \draw [in=180, out=90, ledge] (tl) to (tl);
        \draw [in=0, out=90, ledge] (bl) to (bl);
        \draw [in=0, out=-90, ledge] (br) to (br);
    },
    s/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m s$};

        \node [node, fill=yes] at (0, -1) {};
        \node [node, fill=maybe] at (1, 0) {};
        \node [node, fill=maybe] at (1, -1) {};
    },
    C/.pic={
        \pic {nodes};
        \draw [opacity=0] (tl.north) -- (bl.north) node [varname] {$\m C$};
        \node [node, fill=maybe] at (1, 0) {};
        \node [node, fill=maybe] at (1, -1) {};

        \draw [in=180, out=90, ledge, draw=yes] (tl) to (tl);
        \draw [in=0, out=90, ledge, draw=maybe] (bl) to (bl);
        \draw [in=0, out=-90, ledge, draw=maybe] (br) to (br);

        \draw [dedge, draw=maybe] (tl) -- (bl);
        \draw [dedge, draw=maybe] (tl) -- (br);
    },
    C2/.pic={
        \node [node, fill=yes] (tl) at (0, 0) {};
        \node [node, fill=no, opacity=0] (tr) at (1, 0) {};
        \node [node, fill=no] (bl) at (0, -1) {};
        \node [node, fill=no, opacity=0] (br) at (1, -1) {};
        \node [node, fill=yes] (bm) at (1, -0.5) {};

        \begin{scope}[on background layer]
            \node [object, fit=(tr) (br)] {};
            \node [object, fit=(tl)] {};
            \node [object, fit=(bl)] {};
        \end{scope}

        \draw [in=180+22.5, out=90+22.5, ledge, draw=yes] (tl) to (tl);
        \draw [in=0+22.5, out=-90+22.5, ledge, draw=yes] (bm) to (bm);

        \draw [dedge] (tl) -- (bm);
    },
    model/.pic={
        \node (img) {Image};
        \node (detect) [params, right = 5 mm of img, text width=1.6cm, align=center] {R-CNN};
        \node (l2) [no params, right = 3 mm of detect] {\tiny L2 norm};

        \node (quest) [below = 2 cm of img] {Question};
        \node (embed) [params, text width=1.6cm, align=center] at (detect |- quest) {Embedding};
        \node (rnn) [params, align=center] at (l2 |- embed) {GRU};

        \coordinate (atttop) at ($(l2)!0.25!(rnn)$);
        \coordinate (attmid) at ($(l2)!0.5!(rnn)$);
        \coordinate (attbottom) at ($(l2)!0.75!(rnn)$);
        \coordinate (attmid) at ($(l2)!0.5!(rnn)$);
        \node (attfuse) [no params, right = 7 mm of attmid] {\LARGE$\diamond$};
        \node (attw) [w, right = 2 mm of attfuse] {w};
        \coordinate (softpos) at (attw |- atttop);
        \node (softmax) [no params, right = 7 mm of softpos] {\tiny softmax};
        \node (sum) [no params] at (softmax |- l2) {\tiny$\sum$};

        \coordinate (wq) at (sum.east |- rnn);
        \coordinate (classmiddle) at (sum |- attmid);
        \node (classfuse) [no params, right = 8 mm of classmiddle] {\LARGE$\diamond$};
        \node (classadd) [no params, right = 2 mm of classfuse, draw=red] {\tiny $+$};
        \node (classbn) [params, right = 2 mm of classadd] {\scriptsize BN};
        \node (class) [w, right = 2 mm of classbn] {w};
        \node (classsoft) [no params, right = 2 mm of class] {\tiny softmax};
        \node (end) [right = 2 mm of classsoft] {};

        \node (abovesum) [above = 7 mm of sum] {};
        \node (count) [params, draw=red] at ([xshift=3mm]abovesum) {Count};
        \node (bn) [params, draw=red] at (classadd |- atttop) {\scriptsize BN};
        \node (relu) [no params, draw=red] at (classadd |- sum) {\tiny ReLU};


        \draw [thick, sedge] (img) to ([xshift=-1mm]detect.west);
        \draw [sedge] (detect) to (l2) to (sum);
        \draw [thick, sedge] (quest) to ([xshift=-1mm]embed.west);
        \draw (embed) to (rnn) to (wq);
        \draw (classfuse) to (classadd) to (classbn) to (class) to (classsoft) [sedge] to (end);
        \draw [ledge, out=-45, in=-135, looseness=4] (rnn) to (rnn);

        \draw [sedge] (l2.east) to [out=0, in=90] node [pos=0.5, w] {w} (attfuse);
        \draw [sedge] (rnn.east) to [out=0, in=-90] node [pos=0.5, w] {w} (attfuse);
        \draw (attfuse) to (attw);
        \draw ([yshift=0.3mm]attw.east) to [out=0, in=-90] ([xshift=-0.3mm]softmax.south);
        \draw ([yshift=-0.3mm]attw.east) to [out=0, in=-90] ([xshift=0.3mm]softmax.south);
        \draw [sedge] ([xshift=-0.3mm]softmax.north) to ([xshift=-0.3mm]sum.south);
        \draw [sedge] ([xshift=0.3mm]softmax.north) to ([xshift=0.3mm]sum.south);

        \draw [sedge] (sum) to [out=0, in=90] node [pos=0.5, w] {w} (classfuse);
        \draw [sedge] (wq) to [out=0, in=-90] node [pos=0.5, w] {w} (classfuse);

        \draw [color=red] (count) to [out=0, in=90] node [pos=0.5, color=black, draw=red, w] {w} (relu);
        \draw [color=red] (relu) to (bn) [sedge] to (classadd);

        \begin{scope}[on background layer]
            \draw [sedge, color=red] ([yshift=0.3mm]attw.east) to [out=0, in=180, looseness=0.8] node [pos=0.7, color=black, draw=red, no params] {\small$\sigma$} ([yshift=-0.3mm]count.west);
            \draw [sedge, color=red] ([xshift=-0.4mm, yshift=-0.4mm]detect.north east) to [out=45, in=180, looseness=0.8] node [pos=0.5, above, rotate=13] {\tiny bounding boxes only} ([yshift=0.3mm]count.west);
            \coordinate (crossmid) at ($(attw)!0.4!(count)$);
            \node [fill=white, inner sep=0.8mm, text width=1cm] at (crossmid |- l2) { };
        \end{scope}

    },
}
\makeatother



==> chapters/learn-to-permute/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{Figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Appendix reference, lower-case.
\def\appref#1{Appendix~\ref{#1}}
% Subsection reference, lower-case.
\def\subsecref#1{subsection~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{Algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
% Reference to a table, lower-case.
\def\tabref#1{Table~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Tabref#1{Table~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> chapters/learn-to-permute/tikz_commands.tex <==
\usepackage{tikz}
\usepackage{xcolor}

\usetikzlibrary{shapes, backgrounds, fit, calc, positioning}

\tikzset{
    every picture/.append style={x=5mm, y=5mm},
    box/.style={rectangle,draw=black,thick, minimum size=5mm},
    object/.style={draw, dotted, inner sep=0.3em, fill=green!10},
    desc/.style={rectangle},
    sedge/.style={->, >=stealth},
    varname/.style={midway, above, opacity=1},
    overview/.pic = {
        \pic at (0, 0) {fv};
        \pic at (6, 0) {ordercost};
        \pic at (12, 0) {total cost};
        \pic at (6, -5) {p progression};
        \pic at (19, -5) {result};

        \node [desc] at (0, -3.1) {$\mX$};
        \node [desc] at (7, -3.1) {$\mC$};

        \draw [sedge] (1, -1) -- (4, -1) node [varname, desc, inner sep=3] {$F$} node [midway, below, scale=0.7, inner sep=3] {(learnable)};
        \draw [sedge] (9, -1) -- (10.75, -1) {};
        \draw [sedge, purple, shorten <= 2mm] (c) to[out=-90, in=90, looseness=1.8] (0to1);
        \draw [sedge, purple, shorten <= 2mm] (c) to[out=-90, in=90, looseness=1.8] (1to2);

        \begin{scope}[on background layer]
            \node [object, fit=(p2) (fv result)] {};
        \end{scope}
    },
    result/.pic = {
        \node (dot) at (0, -1) {$\cdot$};
        \pic at (1, 0) {fv};
        \node [desc] at (1, -3.2) {$\mX$};
        \node (eq) at (2.5, -1) {$=$};
        \pic at (4, 0) {fv result};
        \node [desc] at (4, -3.2) {$\mY$};
    },
    p progression/.pic = {
        \pic (p0) at (0, 0) {p0};
        \pic (p1) at (5, 0) {p1};
        \begin{scope}[local bounding box=p2]
            \pic (p2) at (10, 0) {p2};
        \end{scope}

        \node at (-4.2, -0.5) {improve permutation};
        \node at (-4.2, -1.5) {by minimising cost:};

        \draw [sedge] (3, -1) -- (4, -1) node [midway] (0to1) {};
        \draw [sedge] (8, -1) -- (9, -1) node [midway] (1to2) {};

        \node [desc] at (1, -3.1) {$\mP^{(0)}$};
        \node [desc] at (6, -3.1) {$\mP^{(1)}$};
        \node [desc] at (11, -3.1) {$\mP^{(T)}$};
    },
    total cost/.pic = {
        \node [box, fill=black!10, draw=white, inner sep=3] (c) at (0, -1) {$c(\mP)$};
        \node [purple] at (1.75, -3) {$- \frac{\partial c(\mP)}{\partial \mP}$};
        \node at (5.5, -0.5) {function to measure cost};
        \node at (5.5, -1.5) {of permutation with};
    },
    ordercost/.pic = {
        \pic at (-1.33, 0) {fv2};
        \pic at (0, 1.33) {fvT};

        \node [box] at (0, 0) {};
        \node [box, fill=blue!40] at (1, 0) {$<$};
        \node [box, fill=blue!40] at (2, 0) {$<$};
        \node [box, fill=red!40] at (0, -1) {$>$};
        \node [box] at (1, -1) {};
        \node [box, fill=red!40] at (2, -1) {$>$};
        \node [box, fill=red!40] at (0, -2) {$>$};
        \node [box, fill=blue!40] at (1, -2) {$<$};
        \node [box] at (2, -2) {};
    },
    p0/.pic = {
        \node [box, fill=black!33] at (0, 0) {};
        \node [box, fill=black!33] at (1, 0) {};
        \node [box, fill=black!33] at (2, 0) {};
        \node [box, fill=black!33] at (0, -1) {};
        \node [box, fill=black!33] at (1, -1) {};
        \node [box, fill=black!33] at (2, -1) {};
        \node [box, fill=black!33] at (0, -2) {};
        \node [box, fill=black!33] at (1, -2) {};
        \node [box, fill=black!33] at (2, -2) {};
    },
    p1/.pic = {
        \node [box, fill=black!86] at (0, 0) {};
        \node [box, fill=black!14] at (1, 0) {};
        \node [box, fill=black!0] at (2, 0) {};
        \node [box, fill=black!0] at (0, -1) {};
        \node [box, fill=black!12] at (1, -1) {};
        \node [box, fill=black!88] at (2, -1) {};
        \node [box, fill=black!14] at (0, -2) {};
        \node [box, fill=black!75] at (1, -2) {};
        \node [box, fill=black!13] at (2, -2) {};
    },
    p2/.pic = {
        \node [box, fill=black!100] at (0, 0) {};
        \node [box, fill=black!0] at (1, 0) {};
        \node [box, fill=black!0] at (2, 0) {};
        \node [box, fill=black!0] at (0, -1) {};
        \node [box, fill=black!0] at (1, -1) {};
        \node [box, fill=black!100] at (2, -1) {};
        \node [box, fill=black!0] at (0, -2) {};
        \node [box, fill=black!100] at (1, -2) {};
        \node [box, fill=black!0] at (2, -2) {};
    },
    fv/.pic = {
        \node [box, fill=white] at (0, 0) {1};
        \node (fv) [box, fill=white] at (0, -1) {3};
        \node [box, fill=white] at (0, -2) {2};
    },
    fv result/.pic = {
        \node [box, fill=white] at (0, 0) {\textbf{1}};
        \node (fv result) [box, fill=white] at (0, -1) {\textbf{2}};
        \node [box, fill=white] at (0, -2) {\textbf{3}};
    },
    fv2/.pic = {
        \node (x) [box, fill=white, draw=white] at (0, 0) {1};
        \node (fv) [box, fill=white, draw=white] at (0, -1) {3};
        \node (z) [box, fill=white, draw=white] at (0, -2) {2};
        \draw (x.north east) -- (z.south east);
%        \draw (x.north west) -- (x.north east);
%        \draw ($(x.south east)!0.5!(fv.north east)$) -- ($(x.south west)!0.5!(fv.north west)$);
%        \draw ($(fv.south east)!0.5!(z.north east)$) -- ($(fv.south west)!0.5!(z.north west)$);
%        \draw (z.south west) -- (z.south east);
    },
    fvT/.pic = {
        \node (a) [box, fill=white, draw=white] at (0, 0) {1};
        \node (b) [box, fill=white, draw=white] at (1, 0) {3};
        \node (c) [box, fill=white, draw=white] at (2, 0) {2};
        \draw (a.south west) -- (c.south east);
        %\draw (a.north west) -- (a.south west);
        %\draw ($(a.north east)!0.5!(b.north west)$) -- ($(a.south east)!0.5!(b.south west)$);
        %\draw ($(b.north east)!0.5!(c.north west)$) -- ($(b.south east)!0.5!(c.south west)$);
        %\draw (c.north east) -- (c.south east);
    },
    arch classify/.pic = {
        \node (open) {\rotatebox{-90}{$\Bigg\{$}};
        \node [below = -2mm of open] (tiles) {\includegraphics[height=4cm]{analysis/example-mnist-2}};
        \node [below = -2mm of tiles] (close) {\rotatebox{-90}{$\Bigg\}$}};

        \node (cnn1) [fill=yellow!10, trapezium, trapezium angle=80, minimum width=10mm, thick, draw, anchor=north, shape border rotate=270] at (4, -0.75) {CNN};
        \node (cnn2) [fill=yellow!10, trapezium, trapezium angle=80, minimum width=10mm, draw, anchor=north, shape border rotate=270, text=white, dashed] at (4, -2.625) {CNN};
        \node (cnn3) [fill=yellow!10, trapezium, trapezium angle=80, minimum width=10mm, draw, anchor=north, shape border rotate=270, text=white, dashed] at (4, -4.5) {CNN};
        \node (cnn4) [fill=yellow!10, trapezium, trapezium angle=80, minimum width=10mm, draw, anchor=north, shape border rotate=270, text=white, dashed] at (4, -6.375) {CNN};

        \node (F box) [rectangle, draw, minimum width=1.5cm, minimum height=3.5cm] at (9, -4.3) {};
        \node (mlp1) [scale=0.8, rectangle, draw, thick, fill=yellow!10] at (9, -2.5) {MLP};
        \node [above = 1mm of mlp1] {$F$};
        \node (mlp2) [scale=0.8, rectangle, draw, dashed, text=white, fill=yellow!10] at (9, -3.5) {MLP};
        \node [] at (9, -4.5) {\vdots};
        \node (mlp3) [scale=0.8, rectangle, draw, dashed, text=white, fill=yellow!10] at (9, -7) {MLP};

        \node (PO box) [rectangle, draw, minimum width=1.5cm, minimum height=2cm, very thick, fill=green!10] at (15.5, -4.3) {\textbf{PO}};

        \node (resnet) [trapezium, trapezium angle=80, minimum width=14mm, thick, draw, anchor=north, shape border rotate=270, fill=yellow!10] at (21, -3.3) {ResNet-18};

        \draw (tiles.east |- cnn1.west) -- (cnn1.west);
        \draw (tiles.east |- cnn2.west) -- (cnn2.west);
        \draw (tiles.east |- cnn3.west) -- (cnn3.west);
        \draw (tiles.east |- cnn4.west) -- (cnn4.west);

        \draw [sedge] (cnn1.east) -- (F box.west |- cnn1);
        \draw [sedge] (cnn2.east) -- (F box.west |- cnn2);
        \draw [sedge] (cnn3.east) -- (F box.west |- cnn3);
        \draw [sedge] (cnn4.east) -- (F box.west |- cnn4);

        \draw [gray] (F box.west |- cnn1) -- ([yshift=0.3mm]mlp1.west);
        \draw [gray] (F box.west |- cnn1) -- ([yshift=-0.3mm]mlp1.west);
        \draw [gray] (F box.west |- cnn1) -- ([yshift=0.3mm]mlp2.west);
        \draw [gray] (F box.west |- cnn2) -- ([yshift=-0.3mm]mlp2.west);
        \draw [gray] (F box.west |- cnn4) -- ([yshift=0.3mm]mlp3.west);
        \draw [gray] (F box.west |- cnn4) -- ([yshift=-0.3mm]mlp3.west);

        \draw [sedge] (F box.east |- cnn2) -- (PO box.west |- cnn2) node [varname] {\tiny $\mC_{\text{row}}$};
        \draw [sedge] (F box.east |- cnn3) -- (PO box.west |- cnn3) node [varname] {\tiny $\mC_{\text{col}}$};

        \draw [sedge] (PO box.east) -- (resnet.west) node [varname] {};

        \draw [sedge] (open.north) to [bend left=20] (PO box.north);

        \draw [sedge] (resnet.east) -- +(1, 0);
    },
    arch sort/.pic = {
        \node (cnn1) [] at (4, -1.75) {0.3};
        \node (cnn2) [] at (4, -3.50) {0.8};
        \node (cnn3) [] at (4, -5.25) {0.7};
        \node (cnn4) [] at (4, -7) {0.1};

        \node [above = 0mm of cnn1] (open) {\rotatebox{-90}{$\Bigg\{$}};
        \node [below = 0mm of cnn4] (close) {\rotatebox{-90}{$\Bigg\}$}};

        \node (a1) [] at (18, -1.75) {0.1};
        \node [] at (18, -3.50) {0.3};
        \node [] at (18, -5.25) {0.7};
        \node (a4) [] at (18, -7) {0.8};

        \node [above = 0mm of a1] {\rotatebox{-90}{$\Bigg[$}};
        \node [below = 0mm of a4] {\rotatebox{-90}{$\Bigg]$}};

        \node (F box) [rectangle, draw, minimum width=1.5cm, minimum height=3.5cm] at (9, -4.3) {};
        \node (mlp1) [fill=yellow!10, rectangle, draw, thick] at (9, -2.5) {\footnotesize MLP};
        \node [above = 1mm of mlp1] {$F$};
        \node (mlp2) [fill=yellow!10, rectangle, draw, dashed, text=white] at (9, -3.5) {\footnotesize MLP};
        \node [] at (9, -4.5) {\Large\vdots};
        \node (mlp3) [fill=yellow!10, rectangle, draw, dashed, text=white] at (9, -7) {\footnotesize MLP};

        \node (PO box) [rectangle, draw, minimum width=1.5cm, minimum height=2cm, very thick, fill=green!10] at (14, -4.3) {PO};

        \draw [sedge] ([xshift=3mm]cnn1.east) -- (F box.west |- cnn1);
        \draw [sedge] ([xshift=3mm]cnn2.east) -- (F box.west |- cnn2);
        \draw [sedge] ([xshift=3mm]cnn3.east) -- (F box.west |- cnn3);
        \draw [sedge] ([xshift=3mm]cnn4.east) -- (F box.west |- cnn4);

        \draw [gray] (F box.west |- cnn1) -- ([yshift=0.3mm]mlp1.west);
        \draw [gray] (F box.west |- cnn1) -- ([yshift=-0.3mm]mlp1.west);
        \draw [gray] (F box.west |- cnn1) -- ([yshift=0.3mm]mlp2.west);
        \draw [gray] (F box.west |- cnn2) -- ([yshift=-0.3mm]mlp2.west);
        \draw [gray] (F box.west |- cnn4) -- ([yshift=0.3mm]mlp3.west);
        \draw [gray] (F box.west |- cnn4) -- ([yshift=-0.3mm]mlp3.west);

        \draw [sedge] (F box.east) -- (PO box.west) node [varname] {\tiny $\mC$};

        \draw [sedge] (PO box.east) -- +(1, 0);

        \draw [sedge] (open.north) to [bend left=25] (PO box.north);
    },
    arch ban/.pic = {
        \node (v) at (0.5, -1.4) {Object proposals};
        \node (q) at (0.5, -2.65) {Question};

        \node (ban box) [rectangle, draw, minimum height = 2.5cm, minimum width = 10cm, thick, fill=blue!7] at (14, -1) {};
        \node [below = 1mm of ban box.south] {BAN};
        \node (glimpse) [rectangle, draw, minimum height = 1cm, align=center, fill=white, inner sep=3] at (7.2, -2) {Attention glimpse};
        \node (glimpse2) [rectangle, draw, minimum height = 1cm, align=center, fill=white, inner sep=3] at (18, -2) {Attention glimpse};
        \node (dot) [right = 0cm of glimpse2, minimum height = 1cm, align=center, text width = 1.2cm] {$\cdots$};
        \node (dot2) [minimum height = 1cm, align=center, text width = 1.2cm] at (20.5, 2.8) {$\cdots$};

        \node (f) [rectangle, draw, minimum height = 8mm, minimum width = 10mm, very thick, fill=green!10, inner sep=4] at (10, 2.8) {$F$ $\to$ \textbf{PO}};
        \node (lstm) [rectangle, draw, minimum height = 8mm, minimum width = 10mm, thick, fill=yellow!10] at (13.5, 2.8) {LSTM};

        \draw [sedge, very thick, densely dotted] ([yshift=8mm]ban box.west) -- ([yshift=8mm] ban box.east) node [pos=0.25] (p1) {} node [pos=0.8] (p2) {} node [pos=0.67] (p3) {};

        \draw [very thick, densely dotted] (glimpse) to[out=90, in=180] (p1);
        \draw [very thick, densely dotted] (glimpse2) to[out=90, in=180] (p2);
        \draw [very thick, densely dotted] (lstm) to[out=0, in=180] (p3);

        \draw [sedge] ([xshift=-3mm]glimpse.north) to[out=90, in=180] ([yshift=-1mm]f.west);
        \draw [sedge] ([xshift=-3mm]glimpse2.north) to[out=90, in=180] ([yshift=-1mm]19.2, 2.8);
        \draw [sedge] (v.north) to[out=90, in=180] ([yshift=1mm]f.west);
        \draw [dotted] ([yshift=1mm]17, 2.8) -- +(0.5, 0);
        \draw [sedge] ([yshift=1mm]17.5, 2.8) -- ([yshift=1mm]19.2, 2.8);
        \draw [sedge] (f) -- (lstm);

        \draw [sedge] (v) -- (ban box.west |- v);
        \draw [sedge] (q) -- (ban box.west |- q);

    },
}
% actual outputs from net trained on three numbers from [0, 1] transferred to the input {1, 3, 2}
%tensor([[[0.3333, 0.3333, 0.3333],
%         [0.3333, 0.3333, 0.3333],
%         [0.3333, 0.3333, 0.3333]]], device='cuda:0')
%tensor([[[0.8639, 0.1261, 0.0006],
%         [0.0005, 0.1190, 0.8707],
%         [0.1356, 0.7549, 0.1287]]],
%       device='cuda:0', grad_fn=<SelectBackward>)
%tensor([[[9.3886e-01, 7.9670e-03, 3.6252e-07],
%         [2.7509e-07, 6.9721e-03, 9.4433e-01],
%         [6.1142e-02, 9.8506e-01, 5.5666e-02]]],
%       device='cuda:0', grad_fn=<SelectBackward>)


==> chapters/learn-to-set/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,amsthm,mathtools}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{Figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Appendix reference, lower-case.
\def\appref#1{Appendix~\ref{#1}}
% Subsection reference, lower-case.
\def\subsecref#1{subsection~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{Algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
% Reference to a table, lower-case.
\def\tabref#1{Table~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Tabref#1{Table~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vbw{{\bm{\bar{w}}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vyp{{\bm{y'}}}
\def\vhy{{\bm{\hat{y}}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mbW{{\bm{\bar{W}}}}
\def\mX{{\bm{X}}}
\def\mvX{{\bm{\vec{X}}}}
\def\mY{{\bm{Y}}}
\def\mhY{{\bm{\hat{Y}}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\def \enc {{g_{\text{enc}}}}
\def \dec {{g_{\text{dec}}}}
\def \Lrepr {{L_{\text{repr}}}}
\def \Lcha {{L_{\text{cha}}}}
\def \Lhun {{L_{\text{hun}}}}
\def \Lset {{L_{\text{set}}}}
\DeclareMathOperator*{\pool}{pool}
\def\vhm{{\bm{\hat{m}}}}
\def\hm{{\hat{m}}}


==> chapters/learn-to-set/poster/tikz.tex <==
%!TEX root = poster.tex

\usepackage{tikz}
\usepackage{xcolor}
\usepackage{gensymb}

\usetikzlibrary{shapes, backgrounds, fit, calc, positioning, arrows.meta, bending}

% colorbrewer colours, taken from https://github.com/vtraag/tikz-colorbrewer/blob/master/colorbrewer.sty because I couldn't get \usetikzlibrary{colorbrewer} to work
\definecolor{RdYlBu-4-1}{RGB}{215,25,28}
\definecolor{RdYlBu-4-2}{RGB}{253,174,97}
\definecolor{RdYlBu-4-3}{RGB}{171,217,233}
\definecolor{RdYlBu-4-4}{RGB}{44,123,182}
\definecolor{Blues-4-1}{RGB}{239,243,255}
\definecolor{Blues-4-2}{RGB}{189,215,231}
\definecolor{Blues-4-3}{RGB}{107,174,214}
\definecolor{Blues-4-4}{RGB}{33,113,181}
\definecolor{Oranges-4-1}{RGB}{254,237,222}
\definecolor{Oranges-4-2}{RGB}{253,190,133}
\definecolor{Oranges-4-3}{RGB}{253,141,60}
\definecolor{Oranges-4-4}{RGB}{217,71,1}
\definecolor{Purples-4-1}{RGB}{242,240,247}
\definecolor{Purples-4-2}{RGB}{203,201,226}
\definecolor{Purples-4-3}{RGB}{158,154,200}
\definecolor{Purples-4-4}{RGB}{106,81,163}

\newcommand{\AxisRotator}[1][rotate=0]{%
    \tikz [x=1.1mm,y=1.1mm,line width=.1ex,>={Latex[length=.3em, bend]},#1] \draw (0,0) arc (-150:170:1);%
}

% https://tex.stackexchange.com/a/66220
\def\centerarc[#1](#2)(#3:#4:#5)% Syntax: [draw options] (center) (initial angle:final angle:radius)
    { \draw[#1] ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5); }

\tikzset{
    every picture/.append style={x=5mm, y=5mm},
    circ/.style={circle, draw=black, fill=black, minimum size=2.5mm, inner sep=0mm},
    box/.style={rectangle,draw=black,thick, minimum size=5mm},
    object/.style={draw, dotted, inner sep=0.3em, fill=black!3, rounded corners=1mm},
    desc/.style={rectangle},
    sedge/.style={->, >=stealth},
    dedge/.style={<->, >=stealth},
    varname/.style={midway, above, opacity=1},
    symmetry/.pic = {
        % \node [scale=0.9] at (6.5, 2) {The Responsibility Problem};

        \pic at (0, 0) {square};
        \begin{scope}[on background layer]
            \node (s1) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic at (13, 0) {square};
        \begin{scope}[on background layer]
            \node (s4) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic [rotate=-30] at (4, -3) {square};
        \begin{scope}[on background layer]
            \node (s2) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic [rotate=-30+90] at (9, -3) {square};
        \begin{scope}[on background layer]
            \node (s3) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \node [above = 0mm of s1, scale=0.7, color=colorTwo] {(a)};
        \node [above = 0mm of s2, scale=0.7, color=colorTwo] {(c)};
        \node [above = 0mm of s3, scale=0.7, color=colorTwo] {(d)};
        \node [above = 0mm of s4, scale=0.7, color=colorTwo] {(b)};

        \draw [sedge] (s1) -- (s4) node [above, midway] {\raisebox{-0.3mm}{\AxisRotator[xscale=-1]} $90\degree$};
        \draw [sedge, draw=red] (s2) -- (s3) node [below, midway] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $\epsilon$} node [above, midway, red, scale=0.4] {discontinuity};
        \draw [sedge] (s1.south) to[bend right] node [below=1.5mm, midway] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $30\degree$} (s2.west);
        \draw [sedge, text width=1.8cm] (s3.east) to[bend right] node [below=4.5mm, pos=0.8] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $60\degree - \epsilon$} (s4.south);
    },
    square/.pic = {
        \node (a) [circ, fill=RdYlBu-4-1] at (-0.8, 0.8) {};
        \node (b) [circ, fill=RdYlBu-4-2] at (0.8, 0.8) {};
        \node (c) [circ, fill=RdYlBu-4-3] at (0.8, -0.8) {};
        \node (d) [circ, fill=RdYlBu-4-4] at (-0.8, -0.8) {};
    },
    square2/.pic = {
        \node (a) [circ, fill=colorOne] at (-0.8, 0.8) {};
        \node (b) [circ, fill=colorOne] at (0.8, 0.8) {};
        \node (c) [circ, fill=colorOne] at (0.8, -0.8) {};
        \node (d) [circ, fill=colorOne] at (-0.8, -0.8) {};
    },
    model/.pic = {
        \pic (inputs) at (0, 0) {inputs};
        \pic (sort) at (8, 0) {sorted};
        \pic [scale=1.25, every node/.style={transform shape}] (output) at (12.75, 0) {output};
        \pic (dweights) at (16, 0) {dweights};
        \pic (cweights) at (20.5, 0) {cweights};

        \node at (2.5, 1.5) {$\mX$};

        \node at (6.35, -1.2) {\scriptsize sort};
        \draw [sedge] (5.6,  0.0) -- (7.2,  0.0);
        \draw [sedge] (5.6,  0.7) -- (7.2,  0.7);
        \draw [sedge] (5.6, -0.7) -- (7.2, -0.7);

        \node at (8.75, 1.5) {$\mvX$};

        \draw [sedge] (10.2,  0.0) -- (12,  0.0);
        \draw [sedge] (10.2,  0.7) -- (12,  0.7);
        \draw [sedge] (10.2, -0.7) -- (12, -0.7);

        \node at (12.75, 1.4) {$\vy$};
        \node at (12.75, -1.35) {\scriptsize dot product};

        \draw [sedge] (15.2,  0.0) -- (13.5,  0.0);
        \draw [sedge] (15.2,  0.7) -- (13.5,  0.7);
        \draw [sedge] (15.2, -0.7) -- (13.5, -0.7);

        \node at (17.0, 1.4) {\scriptsize $f([\scriptscriptstyle 0, \frac{1}{3}, \frac{2}{3}, 1 \displaystyle], \mbW)$};

        \node at (19.2, -1.2) {\scriptsize discretise};

        \node at (23, 1.4) {\scriptsize $f(\cdot, \mbW)$};

        \draw [sedge] (20,  0.0) -- (18.2,  0.0);
        \draw [sedge] (20,  0.7) -- (18.2,  0.7);
        \draw [sedge] (20, -0.7) -- (18.2, -0.7);
    },
    sorted/.pic = {
        \node [box, scale=0.5, fill=Blues-4-4] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-2] at (1.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-1] at (1.5, 0.7) {};

        \node [box, scale=0.5, fill=Oranges-4-4] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-1] at (1.5, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-4] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-2] at (1.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (1.5, -0.7) {};
    },
    inputs/.pic = {
        \node at (0, 0) {$\Bigg\{$};
        \node at (5, 0) {$\Bigg\}$};

        \node [box, scale=0.625, fill=Blues-4-3] at (1, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-4] at (1, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-3] at (1, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-2] at (2, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-2] at (2, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-1] at (2, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-1] at (3, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-3] at (3, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-4] at (3, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-4] at (4, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-1] at (4, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-2] at (4, -0.625) {};
    },
    dweights/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (1.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (1.5, 0.7) {};

        \node [box, scale=0.5, fill=Oranges-4-2] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (1.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.5, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-1] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (1.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-4] at (1.5, -0.7) {};
    },
    cweights/.pic = {
        \draw [very thick] (0, 0) -- (5, 0);
        \draw [very thick, sedge] (0, -1) -- (0, 1.4);
        \draw [very thick] (5, -1) -- (5, 1.4);

        \draw [thick, draw=Blues-4-3] (0, 0.5) -- (2.5, 0.5) -- (5, 0.5);
        \draw [thick, draw=Oranges-4-3] (0, 0) -- (2.5, 1) -- (5, 0);
        \draw [thick, draw=Purples-4-3] (0, -0.5) -- (2.5, -0.5) -- (5, 1);

        \node [circle, scale=0.25, fill=Oranges-4-4] at (0, 0) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (0, 0.5) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (0, -0.5) {};
        \node [circle, scale=0.25, fill=Oranges-4-4] at (1.667, 0.666) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (1.667, 0.5) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (1.667, -0.5) {};
        \node [circle, scale=0.25, fill=Oranges-4-4] at (3.333, 0.666) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (3.333, 0.5) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (3.333, 0) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (5, 1) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (5, 0.5) {};
        \node [circle, scale=0.25, fill=Oranges-4-4] at (5, 0) {};
    },
    output/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3!50!Blues-4-2] at (0, 0.5) {};
        \node [box, scale=0.5, fill=Oranges-4-3!50!Oranges-4-2] at (0, 0.0) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (0, -0.5) {};
    },
    ae/.pic = {
        \pic at (-3, 0) {square2};
        \begin{scope}[on background layer]
            \node (s1) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \node (enc) [trapezium, draw, rotate=-90, inner ysep=3.5mm, trapezium angle=70, fill=colorThree!10] at (3.5, 0) {Encoder};
        \node [box, scale=0.5, fill=Blues-4-3] at (5.5, 0.5) {};
        \node (fv) [box, scale=0.5, fill=Oranges-4-3] at (5.5, 0) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (5.5, -0.5) {};
        \node (dec) [trapezium, draw, rotate=90, inner ysep=3.5mm, trapezium angle=70, fill=colorThree!10] at (7.5, 0) {~~~~MLP~~~~};


        \node [color=colorOne] (i4) at (0,  1.5) {(-1, -1)};
        \node [color=colorOne] (i3) at (0,  0.5) {(~1, -1)};
        \node [color=colorOne] (i2) at (0, -0.5) {(~1, ~1)};
        \node [color=colorOne] (i1) at (0, -1.5) {(-1, ~1)};

        \node [color=RdYlBu-4-1] (o4) at (11,  1.5) {(-1, ~1)};
        \node [color=RdYlBu-4-2] (o3) at (11,  0.5) {(~1, ~1)};
        \node [color=RdYlBu-4-3] (o2) at (11, -0.5) {(~1, -1)};
        \node [color=RdYlBu-4-4] (o1) at (11, -1.5) {(-1, -1)};

        \pic at (14, 0) {square};
        \begin{scope}[on background layer]
            \node (s2) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}


        \draw [sedge] (i1) -- (enc.south |- i1);
        \draw [sedge] (i2) -- (enc.south |- i2);
        \draw [sedge] (i3) -- (enc.south |- i3);
        \draw [sedge] (i4) -- (enc.south |- i4);
        \draw [sedge] (enc) -- (fv);
        \draw [sedge] (fv) -- (dec);
        \draw [sedge] (dec.south |- o1) -- (o1);
        \draw [sedge] (dec.south |- o2) -- (o2);
        \draw [sedge] (dec.south |- o3) -- (o3);
        \draw [sedge] (dec.south |- o4) -- (o4);

    }
}


==> chapters/learn-to-set/table-0.tex <==

\begin{tabular}{ccccc}
\toprule
$\hat{\bm{Y}}^{(5)}$ & $\hat{\bm{Y}}^{(10)}$ & $\hat{\bm{Y}}^{(20)}$ & True $\bm{Y}$ & Baseline\\
\midrule
(-0.80, -0.12, 3.11) & (-2.41, -1.77, 0.27) & (-2.66, 1.82, 0.45) & (-2.82, 1.95, 0.35) & (-2.56, 2.16, 0.35)\\
small gray metal \textcolor{red}{sphere} & small \textcolor{red}{red} metal \textcolor{red}{sphere} & small gray metal cube & small gray metal cube & small \textcolor{red}{red} metal \textcolor{red}{cylinder}\\
(-0.18, -0.33, 3.34) & (-1.98, 1.74, 0.39) & (-2.26, -2.05, 0.29) & (-2.37, -2.18, 0.35) & (-2.52, -2.53, 0.37)\\
\textcolor{red}{large} \textcolor{red}{gray} metal sphere & small \textcolor{red}{gray} metal \textcolor{red}{cube} & small red metal sphere & small red metal sphere & small \textcolor{red}{gray} metal sphere\\
(0.06, 0.85, 3.54) & (-1.60, -0.20, 0.61) & (-1.44, 0.10, 0.61) & (-1.55, 0.22, 0.70) & (-1.58, 1.40, 0.71)\\
large \textcolor{red}{gray} metal sphere & large red metal sphere & large red metal sphere & large red metal sphere & large \textcolor{red}{yellow} metal sphere\\
(0.14, -0.07, 3.36) & (-1.02, 2.44, 0.54) & (-1.03, 2.26, 0.63) & (-1.33, 2.34, 0.70) & (-0.86, 0.28, 0.69)\\
large gray \textcolor{red}{rubber} \textcolor{red}{sphere} & large gray metal cylinder & large gray metal cylinder & large gray metal cylinder & large \textcolor{red}{purple} metal \textcolor{red}{sphere}\\
(0.60, 1.41, 3.45) & (-0.82, -1.96, 0.61) & (-0.69, -2.07, 0.70) & (-0.69, -2.27, 0.70) & (-0.28, -1.84, 0.70)\\
large gray \textcolor{red}{metal} \textcolor{red}{cylinder} & large gray rubber sphere & large gray rubber sphere & large gray rubber sphere & large \textcolor{red}{yellow} rubber sphere\\
(1.03, -0.95, 3.08) & (0.80, -2.50, 0.29) & (0.86, -2.62, 0.30) & (0.95, -2.83, 0.35) & (1.31, -2.55, 0.35)\\
small \textcolor{red}{purple} rubber cube & small yellow rubber cube & small yellow rubber cube & small yellow rubber cube & small \textcolor{red}{gray} rubber cube\\
\bottomrule
\end{tabular}


==> chapters/learn-to-sortpool/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,amsthm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{Figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Appendix reference, lower-case.
\def\appref#1{Appendix~\ref{#1}}
% Subsection reference, lower-case.
\def\subsecref#1{subsection~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{Algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
% Reference to a table, lower-case.
\def\tabref#1{Table~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Tabref#1{Table~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vbw{{\bm{\bar{w}}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vyp{{\bm{y'}}}
\def\vhy{{\bm{\hat{y}}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mbW{{\bm{\bar{W}}}}
\def\mX{{\bm{X}}}
\def\mvX{{\bm{\vec{X}}}}
\def\mY{{\bm{Y}}}
\def\mhY{{\bm{\hat{Y}}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\T}{\mathsf{T}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


==> chapters/learn-to-sortpool/tikz.tex <==
\usepackage{tikz}
\usepackage{xcolor}
\usepackage{gensymb}

\usetikzlibrary{shapes, backgrounds, fit, calc, positioning, arrows.meta, bending}

% colorbrewer colours, taken from https://github.com/vtraag/tikz-colorbrewer/blob/master/colorbrewer.sty because I couldn't get \usetikzlibrary{colorbrewer} to work
\definecolor{RdYlBu-4-1}{RGB}{215,25,28}
\definecolor{RdYlBu-4-2}{RGB}{253,174,97}
\definecolor{RdYlBu-4-3}{RGB}{171,217,233}
\definecolor{RdYlBu-4-4}{RGB}{44,123,182}
\definecolor{Blues-4-1}{RGB}{239,243,255}
\definecolor{Blues-4-2}{RGB}{189,215,231}
\definecolor{Blues-4-3}{RGB}{107,174,214}
\definecolor{Blues-4-4}{RGB}{33,113,181}
\definecolor{Oranges-4-1}{RGB}{254,237,222}
\definecolor{Oranges-4-2}{RGB}{253,190,133}
\definecolor{Oranges-4-3}{RGB}{253,141,60}
\definecolor{Oranges-4-4}{RGB}{217,71,1}
\definecolor{Purples-4-1}{RGB}{242,240,247}
\definecolor{Purples-4-2}{RGB}{203,201,226}
\definecolor{Purples-4-3}{RGB}{158,154,200}
\definecolor{Purples-4-4}{RGB}{106,81,163}

\newcommand{\AxisRotator}[1][rotate=0]{%
    \tikz [x=1.1mm,y=1.1mm,line width=.1ex,>={Latex[length=.3em, bend]},#1] \draw (0,0) arc (-150:170:1);%
}

% https://tex.stackexchange.com/a/66220
\def\centerarc[#1](#2)(#3:#4:#5)% Syntax: [draw options] (center) (initial angle:final angle:radius)
    { \draw[#1] ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5); }

\tikzset{
    every picture/.append style={x=5mm, y=5mm},
    circ/.style={circle, draw=black, fill=black, minimum size=2.5mm, inner sep=0mm},
    box/.style={rectangle,draw=black,thick, minimum size=5mm},
    object/.style={draw, dotted, inner sep=0.3em, fill=black!3, rounded corners=1mm},
    desc/.style={rectangle},
    sedge/.style={->, >=stealth},
    varname/.style={midway, above, opacity=1},
    symmetry/.pic = {
        \pic at (0, 0) {square};
        \begin{scope}[on background layer]
            \node (s1) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic at (13, 0) {square};
        \begin{scope}[on background layer]
            \node (s4) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic [rotate=-30] at (4, -3) {square};
        \begin{scope}[on background layer]
            \node (s2) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic [rotate=-30+90] at (9, -3) {square};
        \begin{scope}[on background layer]
            \node (s3) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \draw [sedge] (s1) -- (s4) node [above, midway] {\raisebox{-0.3mm}{\AxisRotator[xscale=-1]} $90\degree$};
        \draw [sedge, draw=red] (s2) -- (s3) node [below, midway] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $\epsilon$};
        \draw [sedge] (s1.south) to[bend right] node [below=1.5mm, midway] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $30\degree$} (s2.west);
        \draw [sedge, text width=1.8cm] (s3.east) to[bend right] node [below=4.5mm, pos=0.8] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $60\degree - \epsilon$} (s4.south);
    },
    square/.pic = {
        \node (a) [circ, fill=RdYlBu-4-1] at (-0.8, 0.8) {};
        \node (b) [circ, fill=RdYlBu-4-2] at (0.8, 0.8) {};
        \node (c) [circ, fill=RdYlBu-4-3] at (0.8, -0.8) {};
        \node (d) [circ, fill=RdYlBu-4-4] at (-0.8, -0.8) {};
    },
    model/.pic = {
        \pic (inputs) at (0, 0) {inputs};
        \pic (sort) at (8, 0) {sorted};
        \pic [scale=1.25, every node/.style={transform shape}] (output) at (12.75, 0) {output};
        \pic (dweights) at (16, 0) {dweights};
        \pic (cweights) at (20.5, 0) {cweights};

        \node at (2.5, 1.5) {$\mX$};

        \node at (6.35, -1.2) {\scriptsize sort};
        \draw [sedge] (5.6,  0.0) -- (7.2,  0.0);
        \draw [sedge] (5.6,  0.7) -- (7.2,  0.7);
        \draw [sedge] (5.6, -0.7) -- (7.2, -0.7);

        \node at (8.75, 1.5) {$\mvX$};

        \draw [sedge] (10.2,  0.0) -- (12,  0.0);
        \draw [sedge] (10.2,  0.7) -- (12,  0.7);
        \draw [sedge] (10.2, -0.7) -- (12, -0.7);

        \node at (12.75, 1.4) {$\vy$};
        \node at (12.75, -1.35) {\scriptsize dot product};

        \draw [sedge] (15.2,  0.0) -- (13.5,  0.0);
        \draw [sedge] (15.2,  0.7) -- (13.5,  0.7);
        \draw [sedge] (15.2, -0.7) -- (13.5, -0.7);

        \node at (17.0, 1.4) {\scriptsize $f([\scriptscriptstyle 0, \frac{1}{3}, \frac{2}{3}, 1 \displaystyle], \mbW)$};

        \node at (19.2, -1.2) {\scriptsize discretise};

        \node at (23, 1.4) {\scriptsize $f(\cdot, \mbW)$};

        \draw [sedge] (20,  0.0) -- (18.2,  0.0);
        \draw [sedge] (20,  0.7) -- (18.2,  0.7);
        \draw [sedge] (20, -0.7) -- (18.2, -0.7);
    },
    sorted/.pic = {
        \node [box, scale=0.5, fill=Blues-4-4] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-2] at (1.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-1] at (1.5, 0.7) {};

        \node [box, scale=0.5, fill=Oranges-4-4] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-1] at (1.5, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-4] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-2] at (1.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (1.5, -0.7) {};
    },
    inputs/.pic = {
        \node at (0, 0) {$\Bigg\{$};
        \node at (5, 0) {$\Bigg\}$};

        \node [box, scale=0.625, fill=Blues-4-3] at (1, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-4] at (1, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-3] at (1, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-2] at (2, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-2] at (2, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-1] at (2, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-1] at (3, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-3] at (3, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-4] at (3, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-4] at (4, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-1] at (4, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-2] at (4, -0.625) {};
    },
    dweights/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (1.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (1.5, 0.7) {};

        \node [box, scale=0.5, fill=Oranges-4-2] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (1.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.5, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-1] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (1.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-4] at (1.5, -0.7) {};
    },
    cweights/.pic = {
        \draw [very thick] (0, 0) -- (5, 0);
        \draw [very thick, sedge] (0, -1) -- (0, 1.4);
        \draw [very thick] (5, -1) -- (5, 1.4);

        \draw [thick, draw=Blues-4-3] (0, 0.5) -- (2.5, 0.5) -- (5, 0.5);
        \draw [thick, draw=Oranges-4-3] (0, 0) -- (2.5, 1) -- (5, 0);
        \draw [thick, draw=Purples-4-3] (0, -0.5) -- (2.5, -0.5) -- (5, 1);

        \node [circle, scale=0.25, fill=Oranges-4-4] at (0, 0) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (0, 0.5) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (0, -0.5) {};
        \node [circle, scale=0.25, fill=Oranges-4-4] at (1.667, 0.666) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (1.667, 0.5) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (1.667, -0.5) {};
        \node [circle, scale=0.25, fill=Oranges-4-4] at (3.333, 0.666) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (3.333, 0.5) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (3.333, 0) {};
        \node [circle, scale=0.25, fill=Purples-4-4] at (5, 1) {};
        \node [circle, scale=0.25, fill=Blues-4-4] at (5, 0.5) {};
        \node [circle, scale=0.25, fill=Oranges-4-4] at (5, 0) {};
    },
    output/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3!50!Blues-4-2] at (0, 0.5) {};
        \node [box, scale=0.5, fill=Oranges-4-3!50!Oranges-4-2] at (0, 0.0) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (0, -0.5) {};
    },
    ae/.pic = {
        \node (l) at (0, 0) {\includegraphics[width=2cm]{hexagon}};
        \node (enc) [trapezium, draw, rotate=-90, inner ysep=3.5mm, trapezium angle=70] at (3.5, 0) {\scriptsize Encoder};
        \node [box, scale=0.5, fill=Blues-4-3] at (5.5, 0.5) {};
        \node (fv) [box, scale=0.5, fill=Oranges-4-3] at (5.5, 0) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (5.5, -0.5) {};
        \node (dec) [trapezium, draw, rotate=90, inner ysep=3.5mm, trapezium angle=70] at (7.5, 0) {\scriptsize Decoder};
        \node (r) at (11, 0) {\includegraphics[width=2cm]{hexagon}};

        \draw [sedge] ([xshift=-2mm]l.east) -- (enc);
        \draw [sedge] (enc) -- (fv);
        \draw [sedge] (fv) -- (dec);
        \draw [sedge] (dec) -- ([xshift=2mm]r.west);

        \centerarc[<->,>=stealth](0.05,0)(-65+180:-05+180:1.3);
    }
}


==> chapters/learn-to-sortpool/workshop/tikz.tex <==
%!TEX root = poster.tex

\usepackage{tikz}
\usepackage{xcolor}
\usepackage{gensymb}

\usetikzlibrary{shapes, backgrounds, fit, calc, positioning, arrows.meta, bending}

% colorbrewer colours, taken from https://github.com/vtraag/tikz-colorbrewer/blob/master/colorbrewer.sty because I couldn't get \usetikzlibrary{colorbrewer} to work
\definecolor{RdYlBu-4-1}{RGB}{215,25,28}
\definecolor{RdYlBu-4-2}{RGB}{253,174,97}
\definecolor{RdYlBu-4-3}{RGB}{171,217,233}
\definecolor{RdYlBu-4-4}{RGB}{44,123,182}
\definecolor{Blues-4-1}{RGB}{239,243,255}
\definecolor{Blues-4-2}{RGB}{189,215,231}
\definecolor{Blues-4-3}{RGB}{107,174,214}
\definecolor{Blues-4-4}{RGB}{33,113,181}
\definecolor{Oranges-4-1}{RGB}{254,237,222}
\definecolor{Oranges-4-2}{RGB}{253,190,133}
\definecolor{Oranges-4-3}{RGB}{253,141,60}
\definecolor{Oranges-4-4}{RGB}{217,71,1}
\definecolor{Purples-4-1}{RGB}{242,240,247}
\definecolor{Purples-4-2}{RGB}{203,201,226}
\definecolor{Purples-4-3}{RGB}{158,154,200}
\definecolor{Purples-4-4}{RGB}{106,81,163}

\newcommand{\AxisRotator}[1][rotate=0]{%
    \tikz [x=1.1mm,y=1.1mm,line width=.1ex,>={Latex[length=.3em, bend]},#1] \draw (0,0) arc (-150:170:1);%
}

% https://tex.stackexchange.com/a/66220
\def\centerarc[#1](#2)(#3:#4:#5)% Syntax: [draw options] (center) (initial angle:final angle:radius)
    { \draw[#1] ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5); }

\tikzset{
    every picture/.append style={x=5mm, y=5mm},
    circ/.style={circle, draw=black, fill=black, minimum size=2.5mm, inner sep=0mm},
    box/.style={rectangle,draw=black,thick, minimum size=5mm},
    object/.style={draw, dotted, inner sep=0.3em, fill=black!3, rounded corners=1mm},
    desc/.style={rectangle},
    sedge/.style={->, >=stealth},
    dedge/.style={<->, >=stealth},
    varname/.style={midway, above, opacity=1},
    symmetry/.pic = {
        % \node [scale=0.9] at (6.5, 2) {The Responsibility Problem};

        \pic at (0, 0) {square};
        \begin{scope}[on background layer]
            \node (s1) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic at (13, 0) {square};
        \begin{scope}[on background layer]
            \node (s4) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic [rotate=-30] at (4, -3) {square};
        \begin{scope}[on background layer]
            \node (s2) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \pic [rotate=-30+90] at (9, -3) {square};
        \begin{scope}[on background layer]
            \node (s3) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \node [above = 0mm of s1, scale=0.7, color=colorTwo] {(a)};
        \node [above = 0mm of s2, scale=0.7, color=colorTwo] {(c)};
        \node [above = 0mm of s3, scale=0.7, color=colorTwo] {(d)};
        \node [above = 0mm of s4, scale=0.7, color=colorTwo] {(b)};

        \draw [sedge] (s1) -- (s4) node [above, midway] {\raisebox{-0.3mm}{\AxisRotator[xscale=-1]} $90\degree$};
        \draw [sedge, draw=red] (s2) -- (s3) node [below, midway] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $\epsilon$} node [above, midway, red, scale=0.4] {discontinuity};
        \draw [sedge] (s1.south) to[bend right] node [below=1.5mm, midway] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $30\degree$} (s2.west);
        \draw [sedge, text width=1.8cm] (s3.east) to[bend right] node [below=4.5mm, pos=0.8] {\raisebox{-0.5mm}{\AxisRotator[xscale=-1]} $60\degree - \epsilon$} (s4.south);
    },
    square/.pic = {
        \node (a) [circ, fill=RdYlBu-4-1] at (-0.8, 0.8) {};
        \node (b) [circ, fill=RdYlBu-4-2] at (0.8, 0.8) {};
        \node (c) [circ, fill=RdYlBu-4-3] at (0.8, -0.8) {};
        \node (d) [circ, fill=RdYlBu-4-4] at (-0.8, -0.8) {};
    },
    square2/.pic = {
        \node (a) [circ, fill=colorOne] at (-0.8, 0.8) {};
        \node (b) [circ, fill=colorOne] at (0.8, 0.8) {};
        \node (c) [circ, fill=colorOne] at (0.8, -0.8) {};
        \node (d) [circ, fill=colorOne] at (-0.8, -0.8) {};
    },
    model/.pic = {
        \pic (inputs) at (0, 0) {inputs};
        \pic (sort) at (8, 0) {sorted};
        \pic [scale=1.25, every node/.style={transform shape}] (output) at (12.75, 0) {output};
        \pic (dweights) at (16, 0) {dweights};
        \pic (cweights) at (20.5, 0) {cweights};

        \node at (2.5, 1.5) {$\mX$};

        \node at (6.35, -1.2) {\scriptsize sort};
        \draw [sedge] (5.6,  0.0) -- (7.2,  0.0);
        \draw [sedge] (5.6,  0.7) -- (7.2,  0.7);
        \draw [sedge] (5.6, -0.7) -- (7.2, -0.7);

        \node at (8.75, 1.5) {$\mvX$};

        \draw [sedge] (10.2,  0.0) -- (12,  0.0);
        \draw [sedge] (10.2,  0.7) -- (12,  0.7);
        \draw [sedge] (10.2, -0.7) -- (12, -0.7);

        \node at (12.75, 1.4) {$\vy$};
        \node at (12.75, -1.35) {\scriptsize dot product};

        \draw [sedge] (15.2,  0.0) -- (13.5,  0.0);
        \draw [sedge] (15.2,  0.7) -- (13.5,  0.7);
        \draw [sedge] (15.2, -0.7) -- (13.5, -0.7);

        \node at (17.0, 1.4) {\scriptsize $f([\scriptscriptstyle 0, \frac{1}{3}, \frac{2}{3}, 1 \displaystyle], \mbW)$};

        \node at (19.2, -1.2) {\scriptsize discretise};

        \node at (23, 1.4) {\scriptsize $f(\cdot, \mbW)$};

        \draw [sedge] (20,  0.0) -- (18.2,  0.0);
        \draw [sedge] (20,  0.7) -- (18.2,  0.7);
        \draw [sedge] (20, -0.7) -- (18.2, -0.7);
    },
    sorted/.pic = {
        \node [box, scale=0.5, fill=Blues-4-4] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-2] at (1.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-1] at (1.5, 0.7) {};

        \node [box, scale=0.5, fill=Oranges-4-4] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-1] at (1.5, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-4] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-2] at (1.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (1.5, -0.7) {};
    },
    sorted2/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-2] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-1] at (1.0, 0.7) {};\

        \node [box, scale=0.5, fill=Oranges-4-4] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.0, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-4] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (1.0, -0.7) {};
    },
    inputs/.pic = {
        \node at (0, 0) {$\Bigg\{$};
        \node at (5, 0) {$\Bigg\}$};

        \node [box, scale=0.625, fill=Blues-4-3] at (1, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-4] at (1, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-3] at (1, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-2] at (2, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-2] at (2, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-1] at (2, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-1] at (3, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-3] at (3, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-4] at (3, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-4] at (4, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-1] at (4, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-2] at (4, -0.625) {};
    },
    inputs2/.pic = {
        \node at (0, 0) {$\Bigg\{$};
        \node at (5, 0) {$\Bigg\}$};

        \node [box, scale=0.625, fill=Blues-4-3] at (1, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-4] at (1, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-3] at (1, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-2] at (2.5, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-2] at (2.5, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-1] at (2.5, -0.625) {};

        \node [box, scale=0.625, fill=Blues-4-1] at (4, 0.625) {};
        \node [box, scale=0.625, fill=Oranges-4-3] at (4, 0.0) {};
        \node [box, scale=0.625, fill=Purples-4-4] at (4, -0.625) {};
    },
    dweights/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (1.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (1.5, 0.7) {};

        \node [box, scale=0.5, fill=Oranges-4-2] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-3] at (1.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.5, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-1] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (1.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-4] at (1.5, -0.7) {};
    },
    dweights2/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3] at (0.0, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (0.5, 0.7) {};
        \node [box, scale=0.5, fill=Blues-4-3] at (1.0, 0.7) {};

        \node [box, scale=0.5, fill=Oranges-4-2] at (0.0, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-4] at (0.5, 0.0) {};
        \node [box, scale=0.5, fill=Oranges-4-2] at (1.0, 0.0) {};

        \node [box, scale=0.5, fill=Purples-4-1] at (0.0, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (0.5, -0.7) {};
        \node [box, scale=0.5, fill=Purples-4-4] at (1.0, -0.7) {};
    },
    cweights/.pic = {
        \draw [very thick] (0, 0) -- (5, 0);
        \draw [very thick, sedge] (0, -1) -- (0, 1.4);
        \draw [very thick] (5, -1) -- (5, 1.4);

        \draw [thick, draw=Blues-4-3] (0, 0.5) -- (2.5, 0.5) -- (5, 0.5);
        \draw [thick, draw=Oranges-4-3] (0, 0) -- (2.5, 1) -- (5, 0);
        \draw [thick, draw=Purples-4-3] (0, -0.5) -- (2.5, -0.5) -- (5, 1);

        \node [circle, scale=0.35, fill=Blues-4-4] at (0, 0.5) {};
        \node [circle, scale=0.35, fill=Purples-4-4] at (0, -0.5) {};
        \node [circle, scale=0.35, fill=Blues-4-4] at (1.667, 0.5) {};
        \node [circle, scale=0.35, fill=Purples-4-4] at (1.667, -0.5) {};
        \node [circle, scale=0.35, fill=Oranges-4-4] at (0, 0) {};
        \node [circle, scale=0.35, fill=Blues-4-4] at (3.333, 0.5) {};
        \node [circle, scale=0.35, fill=Purples-4-4] at (3.333, 0) {};
        \node [circle, scale=0.35, fill=Oranges-4-4] at (1.667, 0.666) {};
        \node [circle, scale=0.35, fill=Purples-4-4] at (5, 1) {};
        \node [circle, scale=0.35, fill=Blues-4-4] at (5, 0.5) {};
        \node [circle, scale=0.35, fill=Oranges-4-4] at (3.333, 0.666) {};
        \node [circle, scale=0.35, fill=Oranges-4-4] at (5, 0) {};
        },
        cweights2/.pic = {
            \draw [very thick] (0, 0) -- (5, 0);
            \draw [very thick, sedge] (0, -1) -- (0, 1.4);
            \draw [very thick] (5, -1) -- (5, 1.4);
    
            \draw [thick, draw=Blues-4-3] (0, 0.5) -- (2.5, 0.5) -- (5, 0.5);
            \draw [thick, draw=Oranges-4-3] (0, 0) -- (2.5, 1) -- (5, 0);
            \draw [thick, draw=Purples-4-3] (0, -0.5) -- (2.5, -0.5) -- (5, 1);
    
            \node [circle, scale=0.35, fill=Blues-4-4] at (0, 0.5) {};
            \node [circle, scale=0.35, fill=Blues-4-4] at (2.5, 0.5) {};
            \node [circle, scale=0.35, fill=Blues-4-4] at (5, 0.5) {};
            \node [circle, scale=0.35, fill=Purples-4-4] at (0, -0.5) {};
            \node [circle, scale=0.35, fill=Purples-4-4] at (2.5, -0.5) {};
            \node [circle, scale=0.35, fill=Purples-4-4] at (5, 1) {};
            \node [circle, scale=0.35, fill=Oranges-4-4] at (0, 0) {};
            \node [circle, scale=0.35, fill=Oranges-4-4] at (2.5, 1) {};
            \node [circle, scale=0.35, fill=Oranges-4-4] at (5, 0) {};
    },
    output/.pic = {
        \node [box, scale=0.5, fill=Blues-4-3!50!Blues-4-4] at (0, 0.5) {};
        \node [box, scale=0.5, fill=Oranges-4-3!50!Oranges-4-4] at (0, 0.0) {};
        \node [box, scale=0.5, fill=Purples-4-1] at (0, -0.5) {};
    },
    output2/.pic = {
        \node [box, scale=0.5, fill=Blues-4-2] at (0, 0.5) {};
        \node [box, scale=0.5, fill=Oranges-4-3!50!Oranges-4-2] at (0, 0.0) {};
        \node [box, scale=0.5, fill=Purples-4-1!50!white] at (0, -0.5) {};
    },
    ae/.pic = {
        \pic at (-3, 0) {square2};
        \begin{scope}[on background layer]
            \node (s1) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}

        \node (enc) [trapezium, draw, rotate=-90, inner ysep=3.5mm, trapezium angle=70, fill=colorThree!10] at (3.5, 0) {Encoder};
        \node [box, scale=0.5, fill=Blues-4-3] at (5.5, 0.5) {};
        \node (fv) [box, scale=0.5, fill=Oranges-4-3] at (5.5, 0) {};
        \node [box, scale=0.5, fill=Purples-4-3] at (5.5, -0.5) {};
        \node (dec) [trapezium, draw, rotate=90, inner ysep=3.5mm, trapezium angle=70, fill=colorThree!10] at (7.5, 0) {~~~~MLP~~~~};


        \node [color=colorOne] (i4) at (0,  1.5) {(-1, -1)};
        \node [color=colorOne] (i3) at (0,  0.5) {(~1, -1)};
        \node [color=colorOne] (i2) at (0, -0.5) {(~1, ~1)};
        \node [color=colorOne] (i1) at (0, -1.5) {(-1, ~1)};

        \node [color=RdYlBu-4-1] (o4) at (11,  1.5) {(-1, ~1)};
        \node [color=RdYlBu-4-2] (o3) at (11,  0.5) {(~1, ~1)};
        \node [color=RdYlBu-4-3] (o2) at (11, -0.5) {(~1, -1)};
        \node [color=RdYlBu-4-4] (o1) at (11, -1.5) {(-1, -1)};

        \pic at (14, 0) {square};
        \begin{scope}[on background layer]
            \node (s2) [object, fit=(a) (b) (c) (d)] {};
        \end{scope}


        \draw [sedge] (i1) -- (enc.south |- i1);
        \draw [sedge] (i2) -- (enc.south |- i2);
        \draw [sedge] (i3) -- (enc.south |- i3);
        \draw [sedge] (i4) -- (enc.south |- i4);
        \draw [sedge] (enc) -- (fv);
        \draw [sedge] (fv) -- (dec);
        \draw [sedge] (dec.south |- o1) -- (o1);
        \draw [sedge] (dec.south |- o2) -- (o2);
        \draw [sedge] (dec.south |- o3) -- (o3);
        \draw [sedge] (dec.south |- o4) -- (o4);

    }
}

